twoPhaseInterTrackFoam: an OpenFOAM module for Arbitrary Lagrangian/Eulerian Interface Tracking with Surfactants and Subgrid-Scale Modeling

We provide an implementation of the unstructured Finite-Volume Arbitrary Lagrangian / Eulerian (ALE) Interface-Tracking method for simulating incompressible, immiscible two-phase flows as an OpenFOAM module. In addition to interface-tracking capabilities that include tracking of two fluid phases, an implementation of a Subgrid-Scale (SGS) modeling framework for increased accuracy when simulating sharp boundary layers is enclosed. The SGS modeling framework simplifies embedding subgrid-scale profiles into the unstructured Finite Volume discretization. Our design of the SGS model library significantly simplifies adding new SGS models and applying SGS modeling to Partial Differential Equations (PDEs) in OpenFOAM.

==> credit-statement.tex <==
\section*{CRediT author statement}

\begin{description}

\item Tobias Tolle: Conceptualization, Methodology, Software, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization 

\item Dirk Gr\"unding: Conceptualization, Software, Formal analysis, Data Curation, Writing - Original Draft, Writing - Review \& Editing, Visualization 

\item Dieter Bothe: Writing - Review \& Editing, Supervision, Funding acquisition

\item Tomislav Mari\'c: Conceptualization, Methodology, Software, Validation, Investigation, Data Curation, Writing - Original Draft, Writing - Review \& Editing, Visualization, Supervision, Project administration, Funding acquisition

\end{description}


==> sections/mathModel.tex <==
\section{Mathematical model}
\label{sec:mathModel}

The mathematical model for two-phase incompressible isothermal flow of Newtonian fluids consists of describing the region separating the two phases as a sharp interface with no mass. The conservation equations for such a system are described by the incompressible Navier-Stokes equations. Consider the whole domain containing the two phases as $\FullDomain \in \mathbb{\R}^d $ with $d \in \{1,2,3\} $, for times $ t \in [ t_0,t_{\rm end}) \in \R$. The liquid and gas phases, $\LiquidDomain$ and $\GasDomain$ respectively are subsets of $\FullDomain$ as illustrated in figure \{to add\}. The conservation equations are written for each phase and the mass and momentum balances yield
%
\begin{subequations} \label{eq:localContiMomentumBulk}
    \begin{align}
            \nabla \cdot \vel &= 0  &\text{in} \ \ \Omega(t) \backslash \Sigma(t) , \label{eq:localContiBulk} \\
            \partial_t(\rho \vel) + \nabla \cdot (\rho \vel \otimes \vel) &= \nabla \cdot \S + \rho \mathbf{g}   &\text{in} \ \ \Omega( t) \backslash \Sigma(t).
    \end{align}
\end{subequations}
%
Here, $\vel$ is the the continuum mechanical velocity, $\rho$ is the density, and $\mathbf{g}$ is the gravitational acceleration. Furthermore, the stress tensor of the Newtonian fluid is given by
%
\begin{equation}
    \S = - \rm p \mathbf{I} + \S^{\rm visc}    
\end{equation}
%
where $ \S^{\rm visc} \coloneqq \muup (\nabla\vel + \nabla\vel^{\rm T})$ where p is the pressure, $\S^{\rm visc} $ is the viscous stress tensor and $\muup$ is the dynamic viscosity. The bulk equations are complemented by the transmission conditions
%
\begin{align}
       [\![ \vel ]\!] &= 0 , \\
%\begin{equation}
    [\![ \text{p}\mathbf{I} - \S^{\rm visc} ]\!] &= \sigma \kappa \NSigma + \nabla_{\Sigma}\sigma \ \ \text{on}  \ \ \Sigma(t),
%\end{equation}
\end{align}
%
where $\sigma$ is the surface tension coefficient and $\kappa$ is the mean curvature. As a consequence of mass conservation in the absence of phase change i.e., $\Dot{\rm m}=0$ across the interface, the interface displacement is governed by a kinematic condition which is $\rm V_{\Sigma} = \vel \cdot \NSigma$ and is called the speed of normal displacement. 
% In the presence of a solid surface $\partial\Omega$, additional boundary conditions need to be imposed to constrain the liquid wall interaction, namely, the impermeability condition and the Navier Slip boundary condition written as,
% \begin{align}
%     \vel_{\perp} = 0 , \ \  \lambda \vel_{\parallel} + (\S\mathbf{n}_{\partial\Omega})_{\parallel} = 0 \ \ 
%     \text{on}  \ \ \partial\Omega \backslash \Gamma(t)
% \label{eq:wallBCs}
% \end{align}
% Here, as $\lambda \to \infty$, Navier slip reduces to the no-slip boundary condition where the fluid velocity at the wall is equal to zero. In the $\lambda \to 0$ limit, \eqref{eq:wallBCs} reduces to the free slip condition. In the case when a three phase contact line exists defined as $\Gamma(t) \coloneqq \partial\Omega \cap \LiquidDomain(t) \cap \GasDomain$, additional boundary conditions specified to satisfy the considered continuum mechanical model are
% \begin{equation}
%    \rm V_{\Gamma} = \langle \vel,\mathbf{n}_{\Gamma}\rangle , \ \  \theta = f(\rm V_{\Gamma}) \text{on} \ \ \Gamma(t).
% \end{equation}
% At $\Gamma(t)$, the contact angle $\theta$ can depend on contact line speed $rm V_{\Gamma}$ and an overview of different models for $\theta$ and the descritisation of the full model in the ALE framework is given in [cite dirk thesis] and [cite Tukovic2012].  



%%%%%%can be defined using $\cos\theta = - \langle \Nsigma, \mathbf{n}_{\partial\Omega} \rangle$.
